Precise Image Generation on Current Noisy Quantum Computing Devices

The Quantum Angle Generator (QAG) is a new full Quantum Machine Learning model designed to generate accurate images on current Noise Intermediate Scale (NISQ) Quantum devices. Variational quantum circuits form the core of the QAG model, and various circuit architectures are evaluated. In combination with the so-called MERA-upsampling architecture, the QAG model achieves excellent results, which are analyzed and evaluated in detail. To our knowledge, this is the first time that a quantum model has achieved such accurate results. To explore the robustness of the model to noise, an extensive quantum noise study is performed. In this paper, it is demonstrated that the model trained on a physical quantum device learns the noise characteristics of the hardware and generates outstanding results. It is verified that even a quantum hardware machine calibration change during training of up to 8% can be well tolerated. For demonstration, the model is employed in indispensable simulations in high energy physics required to measure particle energies and, ultimately, to discover unknown particles at the Large Hadron Collider at CERN.

==> backup/bib_first_submission.tex <==
%Paper about data encoding
@INPROCEEDINGS{data_encoding,
  author={Weigold, Manuela and Barzen, Johanna and Leymann, Frank and Salm, Marie},
  booktitle={2021 IEEE 18th International Conference on Software Architecture Companion (ICSA-C)}, 
  title={{Expanding Data Encoding Patterns For Quantum Algorithms}}, 
  year={2021},
  volume={},
  number={},
  pages={95-101},
  doi={10.1109/ICSA-C52384.2021.00025}
  }


@misc{controlled_ry,
  doi = {10.48550/ARXIV.2203.04426},
  url = {https://arxiv.org/abs/2203.04426},
  author = {Rakyta, Péter and Zimborás, Zoltán},
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  title = {Efficient quantum gate decomposition via adaptive circuit compression},
  publisher = {arXiv},
  year = {2022},
  copyright = {Creative Commons Attribution Share Alike 4.0 International}
}

  
%Expressibility and entangling capacity paper
@article{expressibility,
	doi = {10.1002/qute.201900070},
	url = {https://doi.org/10.1002\%2Fqute.201900070},
	year = 2019,
	month = {oct},
	publisher = {Wiley},
	volume = {2},
	number = {12},
	pages = {1900070},
	author = {Sukin Sim and Peter D. Johnson and Al{\'{a}}n Aspuru-Guzik},
	title = {Expressibility and Entangling Capability of Parameterized Quantum Circuits for Hybrid Quantum-Classical Algorithms},
	journal = {Advanced Quantum Technologies}
}
  
 %The original paper of the TTN and MERA architecture
@article{TTN_MERA,
	doi = {10.1038/s41534-018-0116-9},
	url = {https://doi.org/10.1038\%2Fs41534-018-0116-9},
	year = 2018,
	month = {dec},
	publisher = {Springer Science and Business Media {LLC}},
 	volume = {4},
 	number = {1},
	author = {Edward Grant and Marcello Benedetti and Shuxiang Cao and others},
	title = {Hierarchical quantum classifiers},
	journal = {npj Quantum Information}
} 
  
 
@article{encoding_classifiers,
	doi = {10.1103/physreva.102.032420},
	url = {https://doi.org/10.1103\%2Fphysreva.102.032420},
	year = 2020,
	month = {sep},
	publisher = {American Physical Society ({APS})},
	volume = {102},
	number = {3},
	author = {Ryan LaRose and Brian Coyle},
	title = {Robust data encodings for quantum classifiers},
	journal = {Physical Review A}
} 
  
@article{angle_encoding_application,
author = {Sierra-Sosa, Daniel and Telahun, Michael and Elmaghraby, Adel},
year = {2020},
month = {01},
pages = {215246-215255},
title = {TensorFlow Quantum: Impacts of Quantum State Preparation on Quantum Machine Learning Performance},
volume = {8},
journal = {IEEE Access},
doi = {10.1109/ACCESS.2020.3040798}
}
  
@article{amplitude_encoding_example,
author = {Ramos-Calderer, Sergi and Pérez-Salinas, Adrián and García-Martín, Diego and Bravo-Prieto, Carlos and Cortada, Jorge and Planagumà, Jordi and Latorre, José},
year = {2019},
month = {12},
pages = {},
title = {Quantum unary approach to option pricing}
}

%our 1D QGAN paper
@misc{1QGAN_hep,
      title={Quantum Machine Learning for {HEP} Detector Simulations}, 
      author={Florian Rehm and Sofia Vallecorsa and Kerstin Borras and Dirk Krücker},
      year={2021},
      url = {http://ceur-ws.org/Vol-3041/363-368-paper-67.pdf},
      publisher = {Conference Proceedings "Distributed Computing and Grid Technologies in Science and Education" (GRID 2021), Dubna, Russia}
}

%our ACM/IEEE QAG paper
@misc{ACM_IEEE_QAG,
  author={{R}ehm, Florian and Vallecorsa, Sofia and Grossi, Michele and Borras, Kerstin and Krücker, Dirk and Schnake, Simon and Verney-Provatas, Alexis-Harilaos},
  booktitle={2022 IEEE/ACM 7th Symposium on Edge Computing (SEC)}, 
  title={Quantum Angle Generator for Image Generation}, 
  year={2022},
  organization={IEEE Computer Society},
  volume={},
  number={},
  pages={425-429},
  doi={10.1109/SEC54971.2022.00064},
  url={https://inspirehep.net/literature/2620987}
}


%state preparation is costly
@article{costly_state_preparation,
author = {Araujo, Israel and Park, Daniel and Petruccione, Francesco and da Silva, Adenilton},
year = {2021},
month = {03},
pages = {},
title = {A divide-and-conquer algorithm for quantum state preparation},
volume = {11},
journal = {Scientific Reports},
doi = {10.1038/s41598-021-85474-1}
}

%max linear state preparation
@article{state_preparation,
  title = {Efficient State Preparation for Quantum Amplitude Estimation},
  author = {Carrera Vazquez, Almudena and Woerner, Stefan},
  journal = {Phys. Rev. Applied},
  volume = {15},
  issue = {3},
  pages = {034027},
  numpages = {12},
  year = {2021},
  month = {Mar},
  publisher = {American Physical Society},
  doi = {10.1103/PhysRevApplied.15.034027},
  url = {https://link.aps.org/doi/10.1103/PhysRevApplied.15.034027}
}

%amplitude encoding costly in state preparation. Angle encoding not
@inproceedings{state_preparation2,
author = {Weigold, Manuela and Barzen, Johanna and Leymann, Frank and Salm, Marie},
title = {Data Encoding Patterns for Quantum Computing},
year = {2020},
isbn = {9781941652169},
publisher = {The Hillside Group},
address = {USA},
booktitle = {Proceedings of the 27th Conference on Pattern Languages of Programs},
articleno = {2},
numpages = {11},
keywords = {speed-up, quantum computing, patterns, quantum algorithms, data encoding},
location = {Virtual Event},
series = {PLoP '20},
doi = {https://dl.acm.org/doi/10.5555/3511065.3511068}
}

%quantum supremacy by entanglement and superposition
@article{quantum_supremacy,
author = {Khrennikov, Andrei},
year = {2021},
month = {04},
pages = {},
title = {Roots of quantum computing supremacy: superposition, entanglement, or complementarity?},
volume = {230},
journal = {The European Physical Journal Special Topics},
doi = {10.1140/epjs/s11734-021-00061-9}
}


%ibmq webpage machines
@misc{ibmq,
   key = {ibmq},
   title={{IBM Quantum Services}},
   publisher={IBM},
   url={https://quantum-computing.ibm.com/services?services=systems},
   urldate = {2022-08-25},
   year = {2022}
}

@article{born_machine,
   title={Differentiable learning of quantum circuit Born machines},
   volume={98},
   ISSN={2469-9934},
   url={http://dx.doi.org/10.1103/PhysRevA.98.062324},
   DOI={10.1103/physreva.98.062324},
   number={6},
   journal={Physical Review A},
   publisher={American Physical Society (APS)},
   author={Liu, Jin-Guo and Wang, Lei},
   year={2018},
   month={Dec} 
   }
   

@INPROCEEDINGS{SPSA,
  author={Alhabsi, Amer H.},
  booktitle={10th International Conference on Information Science, Signal Processing and their Applications (ISSPA 2010)}, 
  title={Improved {SPSA} optimization algorithm requiring a single measurement per iteration}, 
  year={2010},
  volume={},
  number={},
  pages={263-265},
  doi={10.1109/ISSPA.2010.5605476}
}

%IBMq SPSA
@misc{ibmq_SPSA,
      title={{SPSA Optimizer}}, 
      note = {Available at: \url{https://qiskit.org/documentation/stubs/qiskit.algorithms.optimizers.SPSA.html} Accessed in April 2022},
      year = {2022},
      author = {IBMQ}
}


%parameter shift rule
@misc{parameter_shift_rule,
  doi = {10.48550/ARXIV.2107.12390},
  url = {https://arxiv.org/abs/2107.12390},
  author = {Wierichs, David and Izaac, Josh and Wang, Cody and Lin, Cedric Yen-Yu},
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  title = {General parameter-shift rules for quantum gradients},
  publisher = {arXiv},
  year = {2021},
  copyright = {Creative Commons Attribution 4.0 International}
}

%k-means clustering original paper
@ARTICLE{k_means,
  title={A k-means clustering algorithm},
  author={Hartigan, John A and Wong, Manchek A and others},
  journal={Applied statistics},
  volume={28},
  number={1},
  pages={100--108},
  year={1979},
  publisher={USA},
  doi={https://www.jstor.org/stable/2346830?origin=JSTOR-pdf}
  }

%Our ACAT noise study paper
@article{QGAN_ACAT_noise_study,
    doi = {10.1088/1742-6596/2438/1/012093},
    url = {https://dx.doi.org/10.1088/1742-6596/2438/1/012093},
    year = {2023},
    month = {Feb},
    publisher = {IOP Publishing},
    volume = {2438},
    number = {1},
    pages = {012093},
    author = {Kerstin Borras and Su Yeon Chang and Lena Funcke and Michele Grossi and Tobias Hartung and Karl Jansen and Dirk Kruecker and Stefan Kühn and Florian Rehm and Cenk Tüysüz and Sofia Vallecorsa},
    title = {Impact of quantum noise on the training of quantum Generative Adversarial Networks},
    journal = {Journal of Physics: Conference Series},
}


@misc{QGAN_noise_study,
  doi = {10.48550/ARXIV.2201.03068},
  url = {https://arxiv.org/abs/2201.03068},
  author = {Bogdanov, Yu. I. and Bogdanova, N. A. and Fastovets, D. V. and Lukichev, V. F.},
  keywords = {Quantum Physics (quant-ph), FOS: Physical sciences, FOS: Physical sciences},
  title = {Study of the effect of quantum noise on the accuracy of the Schrodinger equation simulation on a quantum computer using the Zalka-Wiesner method},
  publisher = {arXiv},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

%another noise robust QML approach
@misc{noise_robust_circuits,
  doi = {10.48550/ARXIV.2107.10845},
  url = {https://arxiv.org/abs/2107.10845},
  author = {Wang, Hanrui and Ding, Yongshan and others},
  title = {QuantumNAS: Noise-Adaptive Search for Robust Quantum Circuits},
  publisher = {arXiv},
  year = {2021},
  copyright = {Creative Commons Attribution 4.0 International}
}

%discusses also on noisy training
@misc{noise_robust_training,
title={Ro{QNN}: Noise-Aware Training for Robust Quantum Neural Networks},
author={Hanrui Wang and Jiaqi Gu and Yongshan Ding and Zirui Li and Frederic Chong and David Z. Pan and song han},
year={2022},
url={https://openreview.net/forum?id=wwIBobGFj2V}
}
  
%qiskit documentation about noise

@online{qiskit_noise_docu,
  author = {Qiskit},
  title = {Device backend noise model simulations},
  year = 2022,
  url = {https://qiskit.org/documentation/tutorials/simulators/2_device_noise_simulation.html},
  urldate = {2022-08-30}
}
  
 %paper about detector simulations
@Inbook{detector_simulations,
    author="Apostolakis, J.",
    editor="Fabjan, Christian W.
    and Schopper, Herwig",
    title="Detector Simulation",
    bookTitle="Particle Physics Reference Library: Volume 2: Detectors for Particles and Radiation",
    year="2020",
    publisher="Springer International Publishing",
    address="Cham",
    pages="485--531",
    isbn="978-3-030-35318-6",
    doi="10.1007/978-3-030-35318-6_11",
}

@INPROCEEDINGS{Geant4,
    author = "S Agostinelli and others",
    title = "{{GEANT4--a simulation toolkit}}",
    reportNumber = "SLAC-PUB-9350, FERMILAB-PUB-03-339, CERN-IT-2002-003",
    doi = "10.1016/S0168-9002(03)01368-8",
    journal = "Nucl. Instrum. Meth. A",
    volume = "506",
    pages = "250--303",
    year = "2003"
}

%Summary: LHC produces a lot of data, simulations need to much data, we need smarter approaches for the future	
@INPROCEEDINGS{RoadmapHEP,
	author = {Albrecht, Alvesand,  Amadio et al.},
	year = {2019},
	month = {3},
	title = {{A Roadmap for HEP Software and Computing Research and Development for the 2020s}}, 
	volume = {3},
	journal = {Computing and Software for Big Science},
	doi = {10.1007/s41781-019-0031-6}
}

%exploding computational demand for HL-LHC
@article{LHC_computing_demand,
  title={{WLCG data lake prototype for HL-LHC}},
  author={Kadochnikov, Ivan and Bird, Ian and McCance, Gavin and Schovancova, Jaroslava and Girone, Maria and Campana, Simone and Currul, Xavier Espinal},
  journal={Advisory committee},
  pages={127},
  year={2018},
  doi = {https://ceur-ws.org/Vol-2267/509-512-paper-97.pdf}
}

%Example DL usecase in HEP 1
@article{ju2021performance,
  title={Performance of a geometric deep learning pipeline for HL-LHC particle tracking},
  author={Ju, Xiangyang and Murnane, Daniel and Calafiura, Paolo and others},
  journal={The European Physical Journal C},
  volume={81},
  number={10},
  pages={1--14},
  year={2021},
  publisher={Springer},
  doi = {https://doi.org/10.1140/epjc/s10052-021-09675-8}
}

%Example DL usecase in HEP 2
@inproceedings{biscarat2021towards,
  title={{Towards a realistic track reconstruction algorithm based on graph neural networks for the HL-LHC}},
  author={Biscarat, Catherine and Caillou, Sylvain and Rougier, Charline and Stark, Jan and Zahreddine, Jad},
  booktitle={EPJ Web of Conferences},
  volume={251},
  pages={03047},
  year={2021},
  organization={EDP Sciences},
  note = {\url{https://www.epj-conferences.org/articles/epjconf/pdf/2021/05/epjconf_chep2021_03047.pdf}}
}

%Example DL usecase in HEP 3
@article{sela2022deep,
  title={Deep learning study of an electromagnetic calorimeter},
  author={Sela, Elihu and Huang, Shan and Horn, David},
  journal={Algorithms},
  volume={15},
  number={4},
  pages={115},
  year={2022},
  publisher={MDPI},
  doi = {https://doi.org/10.3390/a15040115}
}

@article{calorimeter_cern,
author = {Fabjan, Christian and Gianotti, Fabiola},
year = {2003},
month = {10},
pages = {},
title = {{Calorimetry for Particle Physics}},
volume = {75},
journal = {Reviews of Modern Physics},
doi = {10.1103/RevModPhys.75.1243}
}

%My EnergyGAN training data set
@misc{data_set,
  author       = {Pierini, Maurizio and Zhang, Matt},
  title        = {{CLIC Calorimeter 3D images: Electron showers at Fixed Angle}},
  year         = {2020},
  publisher    = {Zenodo},
  doi          = {10.5281/zenodo.3603122},
  url          = {https://doi.org/10.5281/zenodo.3603122}
}


%My downsampled 8 pixel data set for this study
@misc{quantum_data_set,
  author       = {Florian Rehm},
  title        = {{Downsampled Calorimeter Shower Images to 8 Pixels}},
  year         = {2021},
  publisher    = {Zenodo},
  doi          = {10.5281/zenodo.7025233},
  url          = {https://doi.org/10.5281/zenodo.7025233}
}

%our reduced precision paper
@article{reduced_precision,
   title={{Reduced Precision Strategies for Deep Learning: A High Energy Physics Generative Adversarial Network Use Case}},
   ISBN={9789897584862},
   url={http://dx.doi.org/10.5220/0010245002510258},
   DOI={10.5220/0010245002510258},
   journal={Proceedings of the 10th International Conference on Pattern Recognition Applications and Methods},
   publisher={SCITEPRESS - Science and Technology Publications},
   author={Rehm, Florian and Vallecorsa, Sofia and Saletore, Vikram and others},
   year={2021}
}


%our GRID ML paper
@article{GRID_ML,
   title={BENCHMARK OF GENERATIVE ADVERSARIAL NETWORKS FOR FAST HEP CALORIMETER SIMULATIONS },
   url={http://ceur-ws.org/Vol-3041/310-315-paper-57.pdf},
   journal={Proceedings of the 9th International Conference in Distributed Computing and Grid-technologies in Science and Education (GRID'2021) },
   publisher={Meshcheryakov Laboratory of Information Technologies (MLIT) of the Joint Institute for Nuclear Research (JINR)},
   author={Rehm, Florian and Vallecorsa, Sofia and Borras, Kerstin and Krücker, Dirk},
   year={2021}
}

@misc{optuna,
      title={{Optuna: A Next-generation Hyperparameter Optimization Framework}}, 
      author={Takuya Akiba and Shotaro Sano and Toshihiko Yanase and Takeru Ohta and Masanori Koyama},
      year={2019},
      eprint={1907.10902},
      archivePrefix={arXiv},
      primaryClass={cs.LG},
      doi = {https://arxiv.org/abs/1907.10902},
}

@article{qml_data,
	doi = {10.1038/s41467-021-22539-9},
	url = {https://doi.org/10.1038\%2Fs41467-021-22539-9},
	year = 2021,
	month = {may},
	publisher = {Springer Science and Business Media {LLC}},
  	volume = {12},
	number = {1},
	author = {Hsin-Yuan Huang and Michael Broughton and Masoud Mohseni and others},
	title = {Power of data in quantum machine learning},
	journal = {Nature Communications}
}

%QCNN
@article{QCNN,
	doi = {10.1007/s42484-021-00061-x},
	url = {https://doi.org/10.1007%2Fs42484-021-00061-x},
	year = 2022,
	month = {feb},
	publisher = {Springer Science and Business Media {LLC}},
	volume = {4},
	number = {1},
	author = {Tak Hur and Leeseok Kim and Daniel K. Park},
	title = {Quantum convolutional neural network for classical data classification},
	journal = {Quantum Machine Intelligence}
}

@article{state_prep_amplitude,
	doi = {10.1103/physrevresearch.4.013091},
	url = {https://doi.org/10.1103\%2Fphysrevresearch.4.013091},
	year = 2022,
	month = {feb},
	publisher = {American Physical Society ({APS})},
	volume = {4},
	number = {1},
	author = {Sahel Ashhab},
	title = {Quantum state preparation protocol for encoding classical data into the amplitudes of a quantum information processing register{\textquotesingle}s wave function},
	journal = {Physical Review Research}
}

%Webpage of WLCG
@online{WLCG_webpage,
	url = {https://wlcg-public.web.cern.ch/},
	title = {Worldwide LHC Computing Grid},
	note = {Accessed in June 2022},
	author = {CERN}
}


%a paper which compares LHC data to other big data fields
@misc{bigdata_2021,
  doi = {10.48550/ARXIV.2202.07659},
  url = {https://arxiv.org/abs/2202.07659},
  author = {Clissa, Luca},
  keywords = {Digital Libraries (cs.DL), FOS: Computer and information sciences, FOS: Computer and information sciences},
  title = {Survey of Big Data sizes in 2021},
  publisher = {arXiv},
  year = {2022},
  copyright = {Creative Commons Attribution 4.0 International}
}

%in a github they summarize ML applications in HEP
@misc{ml_hep,
  doi = {10.48550/ARXIV.2102.02770},
  url = {https://arxiv.org/abs/2102.02770},
  author = {Feickert, Matthew and Nachman, Benjamin},
  title = {A Living Review of Machine Learning for Particle Physics},
  publisher = {arXiv},
  year = {2021},
  copyright = {Creative Commons Attribution 4.0 International}
}

@article{qml_hep,
    author = "Wu, Sau Lan and others",
    title = "{Application of Quantum Machine Learning to High Energy Physics Analysis at LHC Using Quantum Computer Simulators and Quantum Computer Hardware}",
    reportNumber = "FERMILAB-CONF-22-331-DI-QIS",
    doi = "10.22323/1.398.0842",
    journal = "PoS",
    volume = "EPS-HEP2021",
    pages = "842",
    year = "2022"
}

@article{no_exponential_speed_up,
	doi = {10.1088/2632-2153/abc17d},
	url = {https://doi.org/10.1088\%2F2632-2153\%2Fabc17d},
	year = 2021,
	month = {mar},
	publisher = {{IOP} Publishing},
	volume = {2},
	number = {1},
	pages = {011003},
	author = {Wen Guan and Gabriel Perdue and Arthur Pesah and Maria Schuld and Koji Terashi and Sofia Vallecorsa and Jean-Roch Vlimant},
	title = {Quantum machine learning in high energy physics},
	journal = {Machine Learning: Science and Technology}
}

@article{NISQ,
	doi = {10.22331/q-2018-08-06-79},
	url = {https://doi.org/10.22331\%2Fq-2018-08-06-79},
	year = 2018,
	month = {aug},
	publisher = {Verein zur Forderung des Open Access Publizierens in den Quantenwissenschaften},
	volume = {2},
	pages = {79},
	author = {John Preskill},
	title = {Quantum Computing in the {NISQ} era and beyond},
	journal = {Quantum}
}


@misc{QML_speedup,
  doi = {10.48550/ARXIV.2207.07250},
  url = {https://arxiv.org/abs/2207.07250},
  author = {Zheng, Han and Li, Zimu and Liu, Junyu and Strelchuk, Sergii and Kondor, Risi},
  title = {On the Super-exponential Quantum Speedup of Equivariant Quantum Machine Learning Algorithms with SU($d$) Symmetry},
  year = {2022},
  copyright = {arXiv.org perpetual, non-exclusive license}
}

%QGAN
@article{QuGAN,
	doi = {10.1103/physreva.98.012324},
	url = {https://doi.org/10.1103\%2Fphysreva.98.012324},
	year = 2018,
	month = {jul},
	publisher = {American Physical Society ({APS})},
	volume = {98},
	number = {1},
	author = {Pierre-Luc Dallaire-Demers and Nathan Killoran},
	title = {Quantum generative adversarial networks},
	journal = {Physical Review A}
}

%QGAN survey
@Article{qgan_survey,
AUTHOR = {Tong Li, Shibin Zhang, Jinyue Xia},
TITLE = {Quantum Generative Adversarial Network: A Survey},
JOURNAL = {Computers, Materials \& Continua},
VOLUME = {64},
YEAR = {2020},
NUMBER = {1},
PAGES = {401--438},
URL = {http://www.techscience.com/cmc/v64n1/39150},
ISSN = {1546-2226},
DOI = {10.32604/cmc.2020.010551}
}


%classical unsolvable problems
@article{unsolvable_problems,
title = {Non-classical computing problems: Toward novel type of quantum computing problems},
journal = {Results in Physics},
volume = {21},
pages = {103536},
year = {2021},
issn = {2211-3797},
doi = {https://doi.org/10.1016/j.rinp.2020.103536},
url = {https://www.sciencedirect.com/science/article/pii/S2211379720319835},
author = {Mohammed Zidan and Hichem Eleuch and Mahmoud Abdel-Aty},
}


@article{Qvariational_autoencoder,
	doi = {10.1088/2058-9565/aada1f},
	url = {https://doi.org/10.1088\%2F2058-9565\%2Faada1f},
	year = 2018,
	month = {sep},
	publisher = {{IOP} Publishing},
	volume = {4},
  	number = {1},
  	pages = {014001},
  	author = {Amir Khoshaman and Walter Vinci and Brandon Denis and Evgeny Andriyash and Hossein Sadeghi and Mohammad H Amin},
  	title = {Quantum variational autoencoder},
  	journal = {Quantum Science and Technology}
}

%Simons paper, but not quantum...
@article{simon_point_clouds,
  title={Generating Calorimeter Showers as Point Clouds},
  author={Schnake, Simon and Kr{\"u}cker, Dirk and Borras, Kerstin},
  note={\url{https://ml4physicalsciences.github.io/2022/files/NeurIPS_ML4PS_2022_77.pdf}}
}














==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


